Snowmass 2021/22 Letter of Interest: A Forward Calorimeter at the LHC

A forward electromagnetic and hadronic calorimeter (FoCal) was proposed as an upgrade to the ALICE experiment, to be installed during LS3 for data-taking in 2027--2029 at the LHC. The FoCal extends the scope of ALICE, which was designed for the comprehensive study of hot and dense partonic matter, by adding new capabilities to explore the small-$x$ parton structure of nucleons and nuclei. The primary objective of the FoCal is high-precision inclusive measurement of direct photons and jets, as well as coincident gamma-jet and jet-jet measurements, in pp and p--Pb collisions. These measurements by FoCal constitute an essential part of a comprehensive small-$x$ program at the LHC down to $x\sim10^{-6}$ and over a large range of $Q^2$ with a broad array of complementary probes, comprising -- in addition to the photon measurements by FoCal and LHCb -- Drell-Yan and open charm measurements planned by LHCb, as well as photon-induced reactions performed by all LHC experiments.

==> Makefile <==
# $Id: Makefile 362 2012-01-24 09:33:40Z loizides $
#############################

TEXSDIR   = ./
PICSDIR   = ./
FILENAME  = focal-loi-main

###

TEXSRCS   = $(shell find $(TEXSDIR) -maxdepth 2 -iname "*.tex")
PICS      = $(shell find $(PICSDIR) -maxdepth 2 -iname "*.eps")
PPICS     = 

VERS      = $(shell fgrep dver $(FILENAME).tex | head -n 1 | cut -d{ -f2 | cut -d} -f1)

ADDFILES  = Makefile

BACKFILES = $(PICS) $(TEXSRCS) 

ARCHFILES = $(TEXSRCS)

SENDFILES = $(TEXSRCS)

PDFPICS   = $(patsubst %.eps,%.pdf,$(PICS))
EPSPICS   = $(patsubst %.pdf,%.eps,$(PPICS))

APICS     = $(shell find */*.tex -exec grep includegraphics "{}" \; | grep -v "%" | cut  -d{ -f2 | cut -d} -f1 )
ALLPICS   = $(patsubst %,./%*,$(APICS)) alicelogo.pdf cernlogo.pdf
APPICS    = $(patsubst %,./%.pdf,$(APICS))
PPPICS    = $(patsubst %,./%.eps,$(APICS))

LATEX	  = latex
PDFTEX    = pdflatex
DVIPS	  = dvips
PS2PDF    = ps2pdf
EPS2EPS   = eps2eps
EPSTOPDF  = epstopdf
THUMBPDF  = thumbpdf
BIBTEX    = bibtex
VPDF	  = evince
#EPSOPTION = --hires --res=600

ARCHTEX   := $(ARCHFILES) alice_public_notes.cls focal-loi.bib Makefile utphys.bst

default:	$(FILENAME).pdf

$(FILENAME):		$(FILENAME).dvi

$(FILENAME).pdf:	$(FILENAME).tex $(TEXSRCS) $(ADDFILES) $(PDFPICS) focal-loi.bib
	$(PDFTEX) 	$(FILENAME)
	$(BIBTEX)       $(FILENAME)
	$(PDFTEX) 	$(FILENAME)
	$(PDFTEX) 	$(FILENAME)

$(FILENAME).dvi:	$(FILENAME).tex $(TEXSRCS) $(ADDFILES)
	$(LATEX) 	$(FILENAME)
	$(BIBTEX)       $(FILENAME)
	$(LATEX) 	$(FILENAME)
	$(LATEX) 	$(FILENAME)

$(FILENAME).ps:		$(FILENAME).dvi $(PICS)
	$(DVIPS) $(FILENAME).dvi -o $(FILENAME).ps


$(FILENAME).tar.gz:	backup

final:	$(FILENAME).tex $(TEXSRCS) $(ADDFILES) $(PDFPICS) 
	$(PDFTEX) 	$(FILENAME)
	$(PDFTEX) 	$(FILENAME)
	$(PDFTEX) 	$(FILENAME)

dvi:	$(FILENAME).dvi

ps:	$(FILENAME).ps

gzip:	ps
	gzip $(FILENAME).ps

pdf:	$(FILENAME).pdf

ps2pdf:	$(FILENAME).dvi
	$(DVIPS) -Ppdf $(FILENAME).dvi -o $(FILENAME).ps
	$(PS2PDF) $(FILENAME).ps

print:  $(FILENAME).ps
	lpr $(FILENAME).ps

vdvi:	$(FILENAME).dvi
	xdvi $(FILENAME).dvi &

vps:	$(FILENAME).ps
	gv $(FILENAME).ps &

vpdf:	$(FILENAME).pdf
	$(VPDF) $(FILENAME).pdf &

edit:
	emacs $(FILENAME).tex

version: pdf
	mv $(FILENAME).pdf $(FILENAME)_${VERS}.pdf

clean:
	rm -f $(FILENAME).dvi $(FILENAME).toc .tmp.eps	\
	$(FILENAME).aux $(FILENAME).out $(FILENAME).tpt \
	$(FILENAME).bbl $(FILENAME).blg $(FILENAME).log \
	$(FILENAME).lof $(FILENAME).lot $(FILENAME).idx \
	$(FILENAME).ind $(FILENAME).ilg $(FILENAME).glo \
	$(FILENAME).blg $(FILENAME).brf missfont.log \
        texput.log core *.aux *.tmp multPbPbNotes.bib
	find $(TEXSDIR) $(PICSDIR) -name "*~" -type f -exec rm -f "{}" \;
	find $(TEXSDIR) $(PICSDIR) -type d -exec chmod 755 "{}" \;
	find $(TEXSDIR) $(PICSDIR) -type f -exec chmod 644 "{}" \;
	find $(TEXSDIR) -name "*.sh" -type f -exec chmod 755 "{}" \;

realclean: clean
	rm -f $(FILENAME).ps.gz $(FILENAME).pdf $(PDFPICS) $(FILENAME).ps $(FILENAME).tar.gz archiv.tar.gz

backup:
	tar -cvzf $(FILENAME)_$(VERS).tar.gz $(FILENAME).tex $(BACKFILES) $(ADDFILES)

arxiv:
	tar -chvzf $(FILENAME)_arxiv_$(VERS).tar.gz $(ARCHTEX) $(ALLPICS) 

.phony: print clean backup arxiv

$(PDFPICS): %.pdf: %.eps
	$(EPS2EPS) $< .tmp.eps && $(EPSTOPDF) $(EPSOPTION) .tmp.eps --outfile=$@ && rm -f .tmp.eps

#$(EPSPICS): %.eps: %.pdf
#	pdftops -eps $< $@

